Research Re: search & Re-search

Search algorithms are often categorized by their node expansion strategy. One option is the depth-first strategy, a simple backtracking strategy that traverses the search space in the order in which successor nodes are generated. An alternative is the best-first strategy, which was designed to make it possible to use domain-specific heuristic information. By exploring promising parts of the search space first, best-first algorithms are usually more efficient than depth-first algorithms. In programs that play minimax games such as chess and checkers, the efficiency of the search is of crucial importance. Given the success of best-first algorithms in other domains, one would expect them to be used for minimax games too. However, all high-performance game-playing programs are based on a depth-first algorithm. This study takes a closer look at a depth-first algorithm, AB, and a best-first algorithm, SSS. The prevailing opinion on these algorithms is that SSS offers the potential for a more efficient search, but that its complicated formulation and exponential memory requirements render it impractical. The theoretical part of this work shows that there is a surprisingly straightforward link between the two algorithms -- for all practical purposes, SSS is a special case of AB. Subsequent empirical evidence proves the prevailing opinion on SSS to be wrong: it is not a complicated algorithm, it does not need too much memory, and it is also not more efficient than depth-first search.

==> ks6.tex <==
%\chapter{Performance}\label{


==> ks7.tex <==
%\chapter{Upper Bounds on Performance}


==> ks9.tex <==
\cleardoublepage
\chapter{Summary}\label{chap:summ}
\markboth{Chapter 7}{Summary}
\subsubsection{Minimax Search}
The research in this thesis originated from a desire to better
understand full-width fixed-depth minimax search algorithm. These
algorithms form the basis of game-playing programs for games such as
chess, Othello and checkers. Minimax search has a wide applicability
in many areas of
artificial intelligence and operations research, but is mostly known
for its successes in game-playing programs. A number of the ideas
originally 
developed in minimax search have also found a use in single agent
search. Examples are enhancements to the A* algorithm and other Branch and
Bound algorithms.

\subsubsection{\SSS}
This work started out as an examination of a best-first minimax
algorithm called 
{\SSS}. The study of {\SSS} has lead to the remarkable result that it
can be reformulated using {\AB}, the standard minimax search algorithm,
plus a form of storage.
In effect, we have formulated a best-first algorithms as a sequence of
depth-first searches. Unlike IDA*---a version of a best-first single
agent algorithm using a sequence of depth-first searches---the {\SSS}
reformulation evaluates exactly the same nodes as the original.

The reformulation is much clearer, making implementation in existing 
game-playing programs trivial.
Due to the complexity of the original formulation of {\SSS}, the
literature is based on analyses and simulations, lacking practical
assessments.
It is said that although {\SSS} builds trees that are smaller than
conventional algorithms, it is impractical, because it uses too much
memory---a common problem of best-first algorithms.

Our tests with three tournament game-playing programs proved this view
perfectly wrong: {\SSS} does not need too much memory, but the trees
that it builds are not smaller than conventional (depth-first)
algorithms. Thus, ironically, there still is no reason to use it in
practical applications like game-playing programs.
% 
% {\SSS} needs storage to build a single max solution tree, which fits
% comfortably in the transposition tables of our three programs.
% Our reformulation shows that {\SSS} can be perfectly emulated using
% null-window {\AB} calls. This concept has been in use for many years in
% algorithms like {\NS}. Furthermore, with move ordering
% enhancements such as iterative deepening and transposition tables,
% depth-first algortihms like {\AB} and {\NS} achieve roughly the same
% number of cutoffs as {\SSS}. The result is that in practice {\SSS}'s
% trees are not smaller.

Our results contradict the conclusions 
of quite a large body of literature based on simulations. The problem
with simulations is that artificial trees differ greatly from the trees
as build by real applications like game-playing programs. The field of
minimax search is fortunate in that it has many high quality
game-playing programs available. To avoid wrong conclusions, these
should be used instead of simulations.

\subsubsection{The {\MT} framework}
% Although the end result is that even in a practical, easy to use,
% reformulation there appears to be no benefit in using {\SSS}, we have
% learned much from this exercise. 
Reformulating {\SSS} using null-window
{\AB} with transposition tables has enhanced our insight into the
nature of minimax search. It suggested the creation of a framework
for best-first full-width fixed-depth minimax algorithms.

Unlike {\SSS}, a new instance of this framework, {\MTDf}, does
out-perform conventional 
{\AB} variants. The performance gain comes at no extra algorithmic
complexity.

\subsubsection{The Minimal Tree}
Game-playing programs typically use many enhancements to the base
algorithms, such as narrow search windows, iterative deepening,
transposition tables and the history heuristic. It is interesting to see
that these techniques enhance the performance of the algorithm to such a
degree, that all mentioned algorithms achieve comparable performance.
In effect, the enhancements have become
more important than the algorithm.

The fact that all our algorithms achieve comparable performance suggests
that they are approaching the theoretical limit on their performance,
Knuth and Moore's minimal tree.

However, the situation is not that simple.
The minimal tree is originally 
defined for a tree of uniform branching factor and
search depth, without transpositions.
Trees generated by practical applications such as game-playing programs
have transpositions and an irregular branching factor.
To deal with these irregularities,
the minimal tree can be redefined as
the tree searched by {\AB} on a perfectly ordered
tree, in other words, {\AB}'s best-case behavior.

The minimal tree is often seen as the limit on the
performance of any full-width fixed-depth algorithm that proves 
the minimax value. In practice, a move causing an {\AB} cutoff may not
represent the smallest cutoff. Other moves may cause a cheaper cutoff.
We have found that the real limit on the performance of minimax
algorithms---the 
real minimal graph---is
at least a factor of 1.25 (for chess) to 2 (for checkers) smaller than
what is generally assumed. This implies that there is more room for
improving full-width fixed-depth minimax algorithms than generally
assumed.
One area for improvement is to make better use of available transpositions.
We propose such an improvement, called ETC.

\subsubsection{Theory and Practice}
Making the step from uniform to real trees has shown us the value of
adequate theoretical concepts. The notions of bounds and solution trees
made efficient reasoning on the behavior of algorithms like {\AB}, {\NS},
{\SSS} and {\MTDf} possible. The lack of adequate notions describing the
structure of trees with irregular branching factors and transpositions
made it much harder to make progress in this field. 

We hope that future research will develop better notions to model these
phenomena. They are essential for making substantial progress in the
quest for better minimax algorithms.


